Learning Cross-modal Contrastive Features for Video Domain Adaptation

Learning transferable and domain adaptive feature representations from videos is important for video-relevant tasks such as action recognition. Existing video domain adaptation methods mainly rely on adversarial feature alignment, which has been derived from the RGB image space. However, video data is usually associated with multi-modal information, e.g., RGB and optical flow, and thus it remains a challenge to design a better method that considers the cross-modal inputs under the cross-domain adaptation setting. To this end, we propose a unified framework for video domain adaptation, which simultaneously regularizes cross-modal and cross-domain feature representations. Specifically, we treat each modality in a domain as a view and leverage the contrastive learning technique with properly designed sampling strategies. As a result, our objectives regularize feature spaces, which originally lack the connection across modalities or have less alignment across domains. We conduct experiments on domain adaptive action recognition benchmark datasets, i.e., UCF, HMDB, and EPIC-Kitchens, and demonstrate the effectiveness of our components against state-of-the-art algorithms.

==> tables/sensitivity.tex <==

% \begin{table}[!t]
% 	\caption{
% 		Performance comparisons on EPIC-Kitchens.
% 	}
% % 	\vspace{1mm}
% 	\label{table:kitchen_sampling}
% 	\small
% 	\centering
% 	\renewcommand{\arraystretch}{1.1}
% 	\setlength{\tabcolsep}{3pt}
% 	\begin{tabular}{lcc}
% 		\toprule
		
% 		Method & Mean & Gain via sampling \\

% % 		\midrule
		
% % 		Source-only & 45.5 &  \\
		
% 		\midrule
		
% 		MM-SADA (w/o sampling) \cite{Munro_cvpr20} & 49.4 & \\
		
% 		MM-SADA (w/ sampling) \cite{Munro_cvpr20} & 49.9 & +0.5 \\
		
% 		\midrule
		
% 		Ours (w/o sampling) & 49.9 &  \\
		
% 		Ours (w/ sampling) & 51.1 & +1.2 \\
		
% % 		\midrule
		
% % 		Supervised-target  & 69.5 & \\
		
% 		\bottomrule
% 	\end{tabular}
% % 	\vspace{-3mm}
% \end{table}

% \begin{table*}[!t]
% 	\caption{
% 		Performance comparisons between our cross-domain contrastive learning and pseudo-label self-training on EPIC-Kitchens. Note that we vary the loss weight $\lambda_d$ for our cross-domain loss and the pseudo-label self-training one $\lambda_p$.
% 	}
% % 	\vspace{1mm}
% 	\label{table:pseudo-label}
% 	\small
% 	\centering
% 	\renewcommand{\arraystretch}{1.1}
% 	\setlength{\tabcolsep}{5pt}
% 	\begin{tabular}{lcccccccc}
% 		\toprule
		
% 		Setting & D2 $\rightarrow$ D1 & D3 $\rightarrow$ D1 & D1 $\rightarrow$ D2 & D3 $\rightarrow$ D2 & D1 $\rightarrow$ D3 & D2 $\rightarrow$ D3 & Mean & Gain\\
		
% 		\midrule
		
% 		Source-only  & 42.5 & 44.3 & 42.0 & 56.3 & 41.2 & 46.5 & 45.5\\
		
% 		\midrule
		
% 		Our Cross-domain ($\lambda_d = 0.75$) & 50.0&	43.0&	48.8&	47.8&	49.9&	56.8&	49.4 & +3.9\\
%         Our Cross-domain ($\lambda_d = 0.1$) & 52.4&	41.7&	47.4&	49.9&	52.8&	56.1&	50.1 & +4.1 \\
%         Our Cross-domain ($\lambda_d = 0.25$) & 46.7&	43.3&	48.1&	47.8&	49.2&	51.4&	47.8 & +2.3 \\
		
% 		\midrule
		
% 		Pseudo-label ($\lambda_p = 0.01$) & 47.7 & 42.8&	47.6&	48.9&	50.4&	56.7	& 49.0 & +3.5 \\
		
% 		Pseudo-label ($\lambda_p = 0.05$) & 48.2 & 43.1 & 48.2 & 48.7 &49.5 & 55.3	& 48.8 & +3.2\\
		
% 		Pseudo-label ($\lambda_p = 0.1$) & 46.8	&43.8	&48.0&	43.1&	45.6&	52.2&	46.6& +1.1 \\
		
% 		Pseudo-label ($\lambda_p = 0.25$) & 45.6&	38.0&	44.6&	35.8&	41.6&	47.0	&42.1& -3.4\\
		
% 		\bottomrule
% 	\end{tabular}
% 	\vspace{-2mm}
% \end{table*}

% \begin{table*}[!h]
% 	\caption{
% 	    \YH{TODO, Donghyun will update new results}
% 		Sensitivity analysis on EPIC-Kitchens. We use a default setting of $\lambda = 0.1$ and $T = 0.8$, and vary each of this parameters while fixing the other one.
% 	}
% % 	\vspace{1mm}
% 	\label{table:analysis}
% 	\small
% 	\centering
% 	\renewcommand{\arraystretch}{1.1}
% 	\setlength{\tabcolsep}{5pt}
% 	\begin{tabular}{lcccccccc}
% 		\toprule
		
% 		Setting & D2 $\rightarrow$ D1 & D3 $\rightarrow$ D1 & D1 $\rightarrow$ D2 & D3 $\rightarrow$ D2 & D1 $\rightarrow$ D3 & D2 $\rightarrow$ D3 & Mean & Gain\\

%         \midrule
		
% 		Source-only  & 42.5 & 44.3 & 42.0 & 56.3 & 41.2 & 46.5 & 45.5 \\
		
% 		Ours ($\lambda = 0.1, T = 0.8$) & 45.3 & 48.3 & 48.4 & 51.2 & 44.0 & 50.5 & 48.0 & +3.1 \\
		
% 		\midrule
		
% 		Ours ($\lambda = 0.25$) & 46.9 & 48 & 47.6 & 49.9 & 43.5 & 50 & 47.7 & +2.8 \\
		
% 		Ours ($\lambda = 0.05$) & 44.6 & 47.5 & 48.4 & 51.1 & 43.7 & 49.5 & 47.5 & +2.6 \\
		
% % 		Ours ($\lambda = 0.01$) \\
		
% 		\midrule
		
% 		Ours ($T = 0.9$) & 45.1 & 47.4 & 48.5 & 52.1 & 44.0 & 49.9 & 47.8 & +2.9\\
		
% 		Ours ($T = 0.6$) &45.5 & 47.8 & 48.0 & 51.6 & 44.5 & 49.6 & 47.8 & +2.9 \\
		
% % 		\midrule
		
% % 		Supervised-target & 62.8 & 62.8 & 71.7 & 71.7 & 74.0 & 74.0 & 69.5 \\
		
% 		\bottomrule
% 	\end{tabular}
% 	\vspace{-3mm}
% \end{table*}

\begin{table}[!h]
	\caption{
	  		Sensitivity analysis on EPIC-Kitchens. We use a default setting of $\lambda = 0.1$ and $T = 0.8$, and vary each of this parameters while fixing the other one.
	}
% 	\vspace{1mm}
	\label{table:analysis}
	\small
	\centering
	\renewcommand{\arraystretch}{1.1}
	\setlength{\tabcolsep}{5pt}
	\begin{tabular}{lcc}
		\toprule
		
		Setting & Mean & Gain\\

        \midrule
		
		Source-only  & 45.5 \\
		
		Ours ($\lambda = 1.25, T = 0.8$) & 51.0 & +5.5 \\
		
		\midrule
		
		Ours ($\lambda = 1.0$) & 50.1 & +4.6 \\
		
		Ours ($\lambda = 1.5$) & 49.5 & +4.0 \\
		
% 		Ours ($\lambda = 0.01$) \\
		
		\midrule
		
		Ours ($T = 0.9$) & 49.6 & +4.1\\
		
		Ours ($T = 0.6$) & 49.8& +4.3 \\
		
% 		\midrule
		
% 		Supervised-target & 62.8 & 62.8 & 71.7 & 71.7 & 74.0 & 74.0 & 69.5 \\
		
		\bottomrule
	\end{tabular}
	\vspace{-3mm}
\end{table}

\paragraph{Sensitivity Analysis.}
To understand the impact on the hyperparameters in our framework, we provide a sensitivity analysis on the loss weight $\lambda$ and the threshold $T$ to compute pseudo labels.
In Table \ref{table:analysis}, similarly we show the source-only model as the reference and our default setting using $\lambda = 0.1$ and $T = 0.8$.
%
Then, in the second group, we fix $T = 0.8$ and vary the $\lambda$ value, while in the third group, we instead fix $\lambda = 0.1$ and vary the $T$ value.
%
Overall, we show that our model performs stably in terms of changing these two hyperparameters, in which all the models still outperform the source-only baseline by more than 2.6\%.
